Divide and Couple: Using Monte Carlo Variational Objectives for Posterior Approximation

Recent work in variational inference (VI) uses ideas from Monte Carlo estimation to tighten the lower bounds on the log-likelihood that are used as objectives. However, there is no systematic understanding of how optimizing different objectives relates to approximating the posterior distribution. Developing such a connection is important if the ideas are to be applied to inference-i.e., applications that require an approximate posterior and not just an approximation of the log-likelihood. Given a VI objective defined by a Monte Carlo estimator of the likelihood, we use a "divide and couple" procedure to identify augmented proposal and target distributions. The divergence between these is equal to the gap between the VI objective and the log-likelihood. Thus, after maximizing the VI objective, the augmented variational distribution may be used to approximate the posterior distribution.

==> framework2.tex <==

\section{The Divide-and-Couple Framework\label{sec:The-Divide-and-Couple-Framework}}

In this section we identify a correspondence between maximizing a
likelihood bound and posterior inference for general non-negative
estimators using a two step ``divide'' and then ``couple'' construction.


\subsection{Divide}

Let $R(\wr)$ be a positive function of $\wr\sim Q(\omega)$ such
that $\E_{Q(\wr)}R(\wr)=p(x)$, i.e., $R$ is an unbiased likelihood
estimator with sampling distribution $Q(\omega)$. The ``divide''
step follows \citep[Claim 1]{Le_2018_AutoEncodingSequentialMonte}:
we can interpret $\E_{Q(\wr)}\log R(\wr)$ as an ELBO by defining
$\pmc$ so that $R\pp{\omega}=\pmc\pp{\omega,x}/\qmc\pp{\omega}$.
That is, $\pmc$ and $\qmc$ ``divide'' to produce $R$. Specifically:

\begin{restatable}{lem1}{trivdivide}\label{lem:lemdivide}Let $\wr$
be a random variable with distribution $Q(\omega)$ and let $R(\wr)$
be a positive estimator such that $\E_{Q(\wr)}R(\wr)=p(x)$. Then
\begin{eqnarray*}
\pmc\pp{\omega,x} & = & Q\pp{\omega}R\pp{\omega}
\end{eqnarray*}
is an unnormalized distribution over $\omega$ with normalization
constant $p(x)$ and $R\pp{\omega}=\pmc\pp{\omega,x}/\qmc\pp{\omega}$
for $Q\pp{\omega}>0$. Furthermore as defined above,
\begin{equation}
\log p(x)=\E_{Q\pp{\wr}}\log R\pp{\wr}+\KL{\qmc(\wr)}{\pmc(\wr|x)}.\label{eq:divide-elbo}
\end{equation}
\end{restatable}While this shows that it is easy to connect a stochastic
likelihood bound to minimizing a KL-divergence, this construction
alone is not useful for probabilistic inference, since neither $\qmc\pp{\omega}$
nor $\pmc\pp{\omega,x}$ make any reference to $z$. Put another way:
Even if $\KL{\qmc(\wr)}{\pmc(\wr|x)}$ is small, so what? This motivates
the coupling step below.\marginpar{} More generally, $\text{\ensuremath{\pmc}}$
is defined by letting $R=d\pmc/dQ$ be the Radon-Nikodym derivative,
a change of measure from $Q$ to $\pmc$; see supplement.

\subsection{Couple}

If the distributions identified in the above lemma are going to be
useful for approximating $p(z|x)$, they must be connected somehow
to $z$. In this section, we suggest \emph{coupling} $\pmc\pp{\omega,x}$
and $p\pp{z,x}$ into some new distribution $\pmc\pp{\omega,z,x}$
with $\pmc(z,x)=p(z,x)$. In practice, it is convenient to describe
couplings via a conditional distribution $a\pp{z|\omega}$ that augments
$\pmc\pp{\omega,x}$. There is a straightforward condition for when
$a$ is valid: for the augmented distribution $\pmc(z,\omega,x)=\pmc(\omega,x)a(z|\omega)$
to be a valid coupling, we require that $\int\pmc(\omega,x)a(z|\omega)d\omega=p(z,x)$.
An equivalent statement of this requirement is as follows.
\begin{defn*}
\label{def:valid-pair}An estimator $R\pp{\omega}$ and a distribution
$a\pp{z|\omega}$ are a \emph{valid estimator-coupling pair} under
distribution $Q(\omega)$ if
\begin{equation}
\E_{Q\pp{\wr}}R(\wr)a(z|\wr)=p(z,x).\label{eq:valid_est_coupling_pair}
\end{equation}
\end{defn*}
The definition implies that $\E_{Q(\wr)}R(\wr)=p(x)$ as may be seen
by integrating out $z$ from both sides. That is, the definition implies
that $R$ is an unbiased estimator for $p\pp x.$

Now, suppose we have a valid estimator/coupling pair and that $R$
is a good (low variance) estimator. How does this help us to approximate
the posterior $p\pp{z|x}$? The following theorem gives the ``divide
and couple'' framework.\footnote{With measures instead of densities would write $Q(z\in B,\omega\in A)=\int_{A}a(z\in B|\omega)dQ(\omega)$
where $a$ is a Markov kernel; see supplement.}

\begin{restatable}{thm1}{divandcouple}\label{thm:div-and-couple}Suppose
that $R\pp{\omega}$ and $a\pp{z|\omega}$ are a valid estimator-coupling
pair under $Q(\omega)$. Then,
\begin{eqnarray}
\qmc\pp{z,\omega} & = & Q\pp{\omega}a\pp{z|\omega},\label{eq:divcouple-q}\\
\pmc\pp{z,\omega,x} & = & Q\pp{\omega}R\pp{\omega}a\pp{z|\omega},\label{eq:divcouple-p}
\end{eqnarray}
are valid distributions and
\begin{equation}
\log p(x)=\E_{Q\pp{\wr}}\log R\pp{\wr}+\KL{\qmc\pp{\zr}}{p\pp{\zr|x}}+\KL{\qmc\pp{\wr|\zr}}{\pmc\pp{\wr|\zr,x}}.\label{eq:div_and_couple_final_decomp}
\end{equation}

\end{restatable}

The final term in \ref{eq:div_and_couple_final_decomp} is a conditional
divergence \citep[Sec. 2.5]{Cover_2006_Elementsinformationtheory}.
This is the divergence over $\omega$ between $\qmc\pp{\omega|z}$
and $\pmc\pp{\omega|z,x}$, averaged over $z$ drawn from $Q\pp z$.
At a high level, this theorem is proved by applying \ref{lem:lemdivide},
using the chain rule of KL-divergence, and simplifying using the fact
that $a$ is a valid coupling. The point of this theorem is: if $R$
is a good estimator, then $\E\log R$ will be close to $\log p\pp x.$
Since KL-divergences are non-negative, this means that the marginal
$Q\pp z$ must be close to the target $p\pp{z|x}.$ A coupling gives
us a way to \emph{transform} $Q\pp{\omega}$ so as to approximate
$p\pp{z|x}.$

To be useful, we need to access $\qmc\pp z$, usually by sampling.
We assume it is possible to sample from $Q\pp{\omega}$ since this
is part of the estimator. The user must supply a routine to sample
from $a(z|\omega$). This is why the ``trivial coupling'' of $a\pp{z|\omega}=p\pp{z|x}$
is not helpful --- if the user could sample from $p\pp{z|x}$, the
inference problem is already solved! Some estimators may be pre-equipped
with a method to approximate $p(z|x)$. For example, in SMC, $\wr$
include particles $z_{i}$ and weights $w_{i}$ such that selecting
a particle in proportion to its weight approximates $p(z|x)$. This
can be seen as a coupling $a(z|\omega)$, which provides an alternate
interpretation of the divergence bounds of \citep{Naesseth_2018_VariationalSequentialMonte}.
The divide and couple framework is also closely related to extended-space
MCMC methods \citep{Andrieu_2010_ParticleMarkovchain}, which also
use extended target distributions that admit $p(z,x)$ as a marginal;
see also \ref{sec:Conclusions}. However, in these methods, the estimators
also seem to come with \textquotedblleft obvious\textquotedblright{}
couplings.  There is no systematic understanding of how to derive
couplings for general estimators.


\subsection{Example\label{subsec:Running-Example-2}}

Consider again the antithetic estimator from \ref{eq:antithetic}.
We saw before that the antithetic estimator gives a tighter variational
bound than naive VI under the distribution in \ref{fig:Naive-VI-running}.
However, that distribution is \emph{less} similar to the target than
the one from naive VI. To reflect this (and match our general notation)
we now\footnote{With this notation, \ref{eq:antithetic} becomes $R=\frac{1}{2}\frac{p\pp{\wr,x}+p\pp{T\pp{\wr},x}}{Q\pp{\wr}}$
where $\wr\sim Q.$ Here and in the rest of this paper, when $p\pp{\cdot,\cdot}$
has two arguments, the first always plays the role of $z$.} write $\wr\sim Q$ (instead of $\zr\sim q$).

Now, we again ask: Since $Q\pp{\omega}$ is a poor approximation of
the target, can we find some other distribution that is a good approximation?
Consider the coupling distribution
\[
a\pp{z|\omega}=\pi\pp{\omega}\ \delta\pp{z-\omega}+\pp{1-\pi\pp{\omega}}\ \delta\pp{z-T\pp{\omega}},\ \ \ \ \pi\pp{\omega}=\frac{p(\omega,x)}{p(\omega,x)+p(T\pp{\omega},x)}.
\]
Intuitively, $a\pp{z|\omega}$ is supported only on $z=\omega$ and
on $z=T\pp{\omega}$, with probability proportional to the target
distribution. It is simple to verify (by substitution, see \ref{claim:antitheticrunningvalidpair}
in supplement) that $R$ and $a$ form a valid estimator-coupling
pair. Thus, the augmented variational distribution is $Q\pp{\omega,z}=Q\pp{\omega}a\pp{z|\omega}.$
To sample from this, draw $\omega\sim Q$ and select $z=\omega$ with
probability $\pi\pp{\omega}$, or $z=T(\omega)$ otherwise. The marginal
$Q(z)$ is shown in \Cref{fig:antithetic-running-samps}. This is
a much better approximation of the target than naive VI.



